Intensional Datatype Refinement

The pattern-match safety problem is to verify that a given functional program will never crash due to non-exhaustive patterns in its function definitions. We present a refinement type system that can be used to solve this problem. The system extends ML-style type systems with algebraic datatypes by a limited form of structural subtyping and environment-level intersection. We describe a fully automatic, sound and complete type inference procedure for this system which, under reasonable assumptions, is worst-case linear-time in the program size. Compositionality is essential to obtaining this complexity guarantee. A prototype implementation for Haskell is able to analyse a selection of packages from the Hackage database in a few hundred milliseconds.

==> benchmarks.tex <==

\section{Benchmark Results By Module}

\subsection{Package \texttt{aeson}}

\input{benchmarks/aeson.tex}

==> canon-env.tex <==
%!TEX root = main.tex

\section{Eliminating Choice of Environment}

The first step is to eliminate the need to find a refinement datatype environment.
Intuitively, when constructing a refinement datatype environment, there is no disadvantage to including as many different refinements as possible.
Therefore, our aim will be to show that there is a canonical refinement environment that includes, in an appropriate sense, all possible refinements of the given underlying datatypes.

\begin{toappendix}

We first show that type assignment is invariant over refinement environments that are essentially the same, formalised using a version of bisimulation lifted (in the obvious way) to environments.

\begin{definition}[Environment Bisimulations]\label{def:bisimulation}
Let two refinement environments be $(\Delta_1 : D_1 \to \Map\ \Con\ (\Seq\ (\Ty\ D_1)),\,r_1)$ and $(\Delta_2: D_2 \to \Map\ \Con\ (\Seq\ (\Ty\  D_2)),\,r_2)$.  
A \emph{bisimulation between $(\Delta_1,r_1)$ and $(\Delta_2,r_2)$} is a relation $R \subseteq D_1 \times D_2$ with the following properties:
\begin{enumerate}[(i)]
  \item If $R(d_1,\,d_2)$ then $r_1(d_1) = r_2(d_2)$.
  \item If $R(d_1,\,d_2)$ and $\Delta_1(d_1)(k)(i)$ is defined, then $\Delta_2(d_2)(k)(i)$ is defined and $\Ty(R)(\Delta_1(d_1)(k)(i),\,\Delta_2(d_2)(k)(i))$.
  \item If $R(d_1,\,d_2)$ and $\Delta_2(d_2)(k)(i)$ is defined, then $\Delta_1(d_1)(k)(i)$ is defined and $\Ty(R)(\Delta_1(d_1)(k)(i),\,\Delta_2(d_2)(k)(i))$.
\end{enumerate}
It is easily verified that there is a largest bisimulation between $(\Delta_1,\,r_1)$ and $(\Delta_2,\,r_2)$, written infix $\approx$ and named \emph{bisimilarity}, that contains all others.
We write $T_1 \approx T_2$ as a convenience for $\Ty(\mathord{\approx})(T_1,T_2)$ and $S_1 \approx S_2$ for $\Sch(\approx)(S_1,\,S_2)$.
\end{definition}

% As we have defined them, bisimulations are not just two-way simulations (as in Lemma \ref{lem:simulation}) only because we are here interested in the relationship between two different refinement type environments.  
Bisimulation is needed because we want to give a guarantee about type assignment in general,
it is not enough to know that one environment merely \emph{simulates} another (in one direction). 
For example, if all that is known is that $\Delta_1$ is \emph{simulated} by $\Delta_2$, in the sense that each datatypes in the former are simulated by some datatype in the latter, it does not follow that $\Delta_2$ may type more expressions.  This is due to the fact that datatypes may appear in arrows contravariantly.

% We write $\Gamma \types_\Delta e : S$ to denote that $\Gamma \types e : S$ is provable under datatype environment $\Delta$.

In what follows, when working in a context with refinement environments $(\Delta_1,r_1)$ and $(\Delta_2,r_1)$ as above and types $T_1 \in D_1$ and $T_2 \in D_2$, we will use $T_1 \approx T_2$ without specifying \emph{which} bisimilarity we are using (i.e. bisimilarity between $(\Delta_1,\,r_1)$ and $(\Delta_2,\,r_2)$) in the expectation that this can be inferred by the reader from the declaration of $T_1$ and $T_2$.
With bisimulations, one can show the following.

\begin{theorem}\label{thm:subtyping-bisim}
  Suppose the following are two refinement datatype environments:
  \[
      (\Delta_1 : D_1 \to \Map\ \Con\ (\Seq\ (\Ty\ D_1)),\,r_1) \qquad
      (\Delta_2 : D_2 \to \Map\ \Con\ (\Seq\ (\Ty\ D_2)),\,r_2)
  \]
  Suppose $T_1,T_2 \in \Ty\ D_1$ and $T_1',T_2' \in \Ty\ D_2$.  If $T_1 \subtype T_2$ and $T_1 \approx T_1'$ and $T_2 \approx T_2'$ then $T_1' \subtype T_2'$.
\end{theorem}
\begin{proof}
  We show $\{(T_1',\,T_2') \mid \exists T_1, T_2 \in \Ty\ D_1.\ T_1 \subtype T_2 \wedge T_1 \approx T_1' \wedge T_2 \approx T_2' \}$ is contained in $\subtype$ by coinduction.
  \begin{description}
    \item[\rlnm{SShape}] Suppose there is $T_1,\,T_2 \in \Ty\ D_1$ such that $T_1 \subtype T_2$ and $T_1 \approx T_1'$ and $T_2 \approx T_2'$ and $r(T_1') \neq r(T_2')$.  Since bisimilar types have the same shape, it follows that $r(T_1) = r(T_1')$ and $r(T_2) = r(T_2')$ which gives the desired contradiction.
    \item[\rlnm{SData}] Suppose there is $T_1,\,T_2 \in \Ty\ D_1$ such that (i) $T_1 \subtype T_2$ and (ii) $T_1 \approx d_1$ and (iii) $T_2 \approx d_2$ and $\Delta_2(d_1)(k)(i)$ is defined.  It follows by definition that $T_1$ is some datatype $d_1'$ and $T_2$ is some datatype $d_2'$.  From (ii) we have that $\Delta_1(d_1')(k)(i)$ is defined and $\Delta_1(d_1')(k)(i) \approx \Delta_2(d_1)(k)(i)$.  From (i) and \rlnm{SData} we have that ($\Delta_1(d_2')(k)(i)$ is defined and) $\Delta_1(d_1')(k)(i) \subtype \Delta_1(d_2')(k)(i)$.  Therefore, by (iii), we have that $\Delta_2(d_2)(k)(i)$ is defined and $\Delta_1(d_2')(k)(i) \approx \Delta_2(d_2)(k)(i)$.  Therefore, we can take as witnesses $\Delta_1(d_1')(k)(i)$ and $\Delta(d_2')(k)(i)$.
    \item[\rlnm{SArrL}] Suppose there is $T_1,\,T_2 \in \Ty\ D_1$ such that $T_1 \subtype T_2$ and $T_1 \approx T_3' \to T_3''$ and $T_2 \approx T_4' \to T_4''$.  It follows by definition that $T_1$ has shape $T_1' \to T_1''$ and $T_2$ has shape $T_2' \to T_2''$.  By \rlnm{SArrL}, $T_2' \subtype T_1'$ and it follows from the definition of $\Ty(\approx)$ that necessarily $T_1' \approx T_3'$ and $T_2' \approx T_4'$ as required.
    \item[\rlnm{SArrR}] Analogously.
  \end{description}
\end{proof}

\begin{corollary}
  Suppose $T,\,T' \in \Ty\ D$ and $T \approx T'$.  Then $T \equiv T'$.
\end{corollary}
\begin{proof}
  For $\mathord{\subtype}$, take $T_1 = T_2 = T_1' = T$ and $T_2' = T'$ in the above theorem.  The $\mathord{\suptype}$ part is symmetric.
\end{proof}


\newcommand{\typesA}{\types_{\Delta_1}}
\newcommand{\typesB}{\types_{\Delta_2}}

\begin{theorem}[(Bisimilarity and type assignment)]
  Suppose the following are two refinement datatype environments:
  \[
    \begin{array}{c}
      (\Delta_1 : D_1 \to \Map\ \Con\ (\Seq\ (\Ty\ D_1)),\,r_1) \\
      (\Delta_2 : D_2 \to \Map\ \Con\ (\Seq\ (\Ty\ D_2)),\,r_2)
    \end{array}
  \]
  and suppose $f : D_1 \to D_2$ has the property that, for all $d \in D_1$, $d \approx f(d)$. Then for all $\Gamma \in \TyEnv\ D_1$ and $T \in \Ty\ D_1$ we have $\Gamma \types e : T$ is derivable in $(\Delta_1,r_1)$ implies $f(\Gamma) \types e : f(T)$ is derivable in $(\Delta_2,r_2)$.
\end{theorem}
\begin{proof}
  The proof is by induction.
  \begin{description}
    \item[\rlnm{TVar}] Suppose $\vv{T} :: \vv{\underline{T}}$ and $x:\forall \vv{\alpha}.\ U \in \Gamma$.  Then $x:\forall \vv{\alpha}.\ f(U) \in f(\Gamma)$.  By definition, $f(U)[\vv{f(T)}/\vv{\alpha}]) = f(U[\vv{T}/\vv{\alpha}])$, so the result follows by \rlnm{TVar}.
    \item[\rlnm{TSub}] Suppose $f(\Gamma) \typesB e : f(T_1)$ and $T_1 \subtype T_2$.  By assumption, $f(T_1) \bisim T_1$ and $f(T_2) \bisim T_2$.  It follows from \ref{thm:subtyping-bisim} that, therefore, $f(T_1) \subtype f(T_2)$.  The result follows from \rlnm{TSub}.
    \item[\rlnm{TCst} \rlnm{TCon}] In these cases, the result follows immediately from the fact that $T$ and $f(T)$ have the same shape.
    \item[\rlnm{TAbs}] Suppose $f(\Gamma) \cup \{x:f(T_1)\} \types e : f(T_2)$ and $T_1 :: \underline{T_1}$ and $x \notin \dom(\Gamma)$.  By definition, $x \notin \dom(f(\Gamma))$ and $f(T_1) :: \underline{T_1}$.  Therefore, the result follows from \rlnm{TTmAbs}.
    \item[\rlnm{TApp}] Suppose $f(\Gamma) \types e_1 : f(T_1) \to f(T_2)$ and $f(\Gamma) \types f(T_1)$.  The results follows immediately from \rlnm{TTmApp}.
    \item[\rlnm{TCase}] Suppose $f(\Gamma) \types e : f(d)$ and, for all $i \in [1..m]$ $f(\Gamma) \cup \vv{x_i : f(\Delta_1(d)(k_i))} \typesB e_i : f(T)$ (*) and $\dom(\Delta_1(d)) \subseteq \{k_1,\ldots,k_m\}$.  Now let $i \in [1..m]$.  Since $d \bisim f(d)$, it follows that $\dom(\Delta_2(f(d))) = \dom(\Delta_1(d))$ and, for each $k_i$ in the domain, $\Delta_1(d)(k_i)(j) \bisim \Delta_2(f(d))(k_j)(j)$ for each $j$ at most the arity of $k_i$.  Therefore, by Theorem \ref{thm:subtyping-bisim} and weakening, it follows from (*) that $f(\Gamma) \cup \vv{x_i : \Delta_2(d)(k_i)} \types e_i : f(T)$.  The desired result then follows from \rlnm{TCase}.
  \end{description}
\end{proof}

\end{toappendix}

\subsection{Canonical Refinement Environment}

We have chosen a treatment of datatypes using environments because it is closest to the way that datatypes are specified in mainstream functional programming languages. 
However, there are features of this representation that are less pleasant to work with, in particular the fact that there are infinitely many presentations of essentially the same datatype, due to the reliance on choosing particular names and the prescence of sharing in the definitions.

To remedy this annoyance, we will concentrate attention on those refinement environments that have a standard choice of names, namely the very same names as the underlying datatype environment.

\begin{definition}[Subrefinement]
A refinement environment $(\Delta : D \to \Map\ \Con\ (\Seq\ (\Ty\ D)),\,r)$ is said to be a \emph{refinement subenvironment} just if $D \subseteq \ul{D}$ and $r : D \to \underline{D}$ is an inclusion.  We write $\SubRefns$ for the collection of all refinement subenvironments.
\end{definition}

Note that subrefinements are not representative of all possible refinement environments (in any sense), since they can essentially only specify at most one refinement of any given underlying datatype.
However, there is a sense in which they represent refinement environments that have this property. 
In particular, they are representative of slice environments.

\begin{definition}[Induced Subrefinement]
Suppose $(\Delta : D \to \Map\ \Con\ (\Seq\ (\Ty\ D)),\,r)$ is a refinement type environment.  Then each refinement datatype $d \in D$ gives rise to a subrefinement $\sub{\subenv{d}{\Delta}}$, \emph{the subrefinement induced by a slice}.  First, we know that the following diagram commutes up to (reverse-) inclusion:
\[
  \begin{tikzcd}
    \subenv{d}{D} \arrow[r,"\subenv{d}{\Delta}"] \arrow[d,"r \restriction \subenv{d}{D}"] & \Map\ \Con\ (\Ty\ \subenv{d}{D}) \arrow[d,"(r \restriction \subenv{d}{D})^*"] \\
    \underline{D} \arrow[r,"\underline{\Delta}"] & \Map\ \Con\ (\Ty\ \underline{D})
  \end{tikzcd}
\]
Second, by local injectivity, $r \restriction \subenv{d}{D}$, the restriction of $r$ to domain $\subenv{d}{D}$, is injective. So, writing $\sub{\subenv{d}{D}}$ for its range, we can define:
\[
  \begin{array}{rcl}
  \sub{\subenv{d}{\Delta}} &:& \sub{\subenv{d}{D}} \to \Map\ \Con\ (\Seq\ (\Ty\ \sub{\subenv{d}{D}})) \\
  \sub{\subenv{d}{\Delta}} &=& (r \restriction \subenv{d}{D})^* \circ \subenv{d}{\Delta} \circ (r \restriction \subenv{d}{D})^{-1} \\ 
  \end{array}
\]
In this way, it is easy to verify that $\sub{\subenv{d}{\Delta}} \in \SubRefns$.
\end{definition}


% It follows that $\underline{\Delta}_d$ is a subrefinement since, for each $d' \in \pol{\ul{d}}$ we have, for some $d' \in D$: 
% \[
%   \begin{array}{rcl}
%   && \iota^*((\Delta \restriction \subenv{d}{\Delta})(\underline{d})) \\
%   &=& \iota^*((\Delta \restriction \subenv{d}{\Delta})(r (\iota_d(d')))) \\
%   &=& \iota^*((r^* \circ \iota_d^* \circ \subenv{d}{\Delta} \circ (r \circ \iota_d)^{-1})(r (\iota_d(d')))) \\
%   &=& \iota^*((r^* \circ \iota_d^*)(\subenv{d}{\Delta}(d')))))
%   \end{array}
% \]
% whose inclusion in $\underline{\Delta}(\iota(\underline{d})) = \underline{\Delta}(\iota(r(\iota_d((d')))))$ follows from (*).  Hence $(\underline{\Delta} \restriction \subenv{d}{\Delta}) \in \SubRefns(\underline{\Delta})$.

The subrefinement induced by a given slice is isomorphic to the slice: the only material difference is a change of datatype names.
Consider the following example.

\begin{example}
  The subrefinement induced by $\mathsf{LATm_0}$ is:\\
  \begin{tabular}{p{.4\columnwidth}p{.6\columnwidth}}
  \begin{lstlisting}
data Arith where
  Lit : Int -> Arith
  Add : Arith
  \end{lstlisting}&
  \begin{lstlisting}
data Lam where
  Cst : Arith -> Lam
  App : Lam -> Lam -> Lam
  \end{lstlisting}
\end{tabular}
  i.e. with the same form as the earlier definition of (= the slice of) $\mathsf{LATm_0}$ but with names taken from the original, underlying datatypes $\mathsf{Lam}$ and $\mathsf{Arith}$.
\end{example}

By restricting attention to subrefinements, we fix a particular choice of names for datatype refinements.  
No generality is lost because every refinement datatype in a given refinement environment has its counterpart in the subrefinement induced by its slice.

Note that it only makes sense to speak of the subrefinement induced by a slice, and not induced to an arbitrary refinement environment, because there is not generally a well-defined subrefinement corresponding to a refinement environment.
When a refinement environment contains more than one refinement of some underlying datatype (as is typical), there is no single induced subrefinement.
For example, the environment $\Delta$ from Example \ref{ex:atms} that defines $\mathsf{ATm}_0$ and $\mathsf{LATm}_0$ does not have an induced subrefinement.
However, all the information relevant to typing that is contained in this environment can be found in the two subrefinements induced by the slices $\subenv{\mathsf{ATm}_0}{\Delta}$ and $\subenv{\mathsf{LATm}_0}{\Delta}$.

\begin{definition}[Canonical Environment]
  Given a family of datatype environments $\Delta_{i \in I} : D_i \to \Map\ \Con\ (\Seq\ (\Ty\ D_i))$ we define their coproduct as the environment:
\[
  \coprod_{i \in I} \Delta_i : \coprod_{i \in I} D_i \to \Map\ \Con\ (\Seq\ (\Ty\ \coprod_{i \in I} D_i))
\]
satisfying $(\coprod_{i \in I} \Delta_i)(\inj_i d) = \inj_i^\dagger (\Delta_i(d))$.  It is worth noting that this ensures $(\coprod_{i \in I} \Delta_i)(\inj_i\ d)(k)(i)$ is defined iff $\Delta_i(d)(k)(i)$ is defined.   Moreover, if each of these environments is a refinement by some $r_i : D_i \to \underline{D}$, then so is the coproduct, as witnessed by the copairing $r : \coprod_{i \in I} D_i \to \underline{D}$:
\[
  r(\inj_i d) = r_i(d)
\]
  We define the \emph{canonical refinement type environment}, written $\canon{\Delta} : \canon{D} \to \Map\ \Con\ (\Seq\ (\Ty\ \canon{D}))$, as the coproduct of all subrefinements of $\ul{\Delta}$.
\end{definition}

By limiting $D_i$ to subrefinement environments, we get the stronger property that $\canon{\Delta}(\inj_i(d))(k) = \inj_i(\ul{\Delta}(d)(k))$ when defined.
We shall refer to this as \emph{compatibility}.

The disjoint collection of all subrefinements, $\canon{\Delta}$, is as good a refinement environment as any other.  Any particular datatype $d$ defined in any particular refinement environment $\Delta$ will find a counterpart in $\sub{\subenv{d}{\Delta}}$ (the subrefinement induced by $\subenv{d}{\Delta}$), which is one of the components of $\canon{\Delta}$.

To be more precise, suppose $\Delta : D \to \Map\ \Con\ (\Seq\ (\Ty\ D)$ is a datatype environment with refinement given by $r$. We can define $f : D \to \canon{D}$ so that $\Gamma \types e : T$ in $\Delta$ implies $f(\Gamma) \types e : f(T)$ in $\canon{\Delta}$.
The action of $f$ is to map each datatype $d \in D$ to $\inj_{\sub{\subenv{d}{\Delta}}}\ r(d)$, i.e. the datatype named by the underlying type of $d$ in the subrefinement induced by its slice.
It follows that, for the purpose of typability, considering $\canon{\Delta}$ suffices:

\begin{theoremrep}
  $\ul{\Delta};\, \Gamma \types m$ is refinement typable iff there is a refinement type environment $\Gamma'$ such that $\canon{\Delta},\,\Gamma \types m : \Gamma'$.
\end{theoremrep}
\begin{proof}
  Suppose $\Delta : D \to \Map\ \Con\ (\Seq\ (\Ty\ D)$ is a datatype environment with refinement given by $r$. We can define $f : D \to \canon{D}$ so that $f(d) \approx d$.  
  To see this, let $f(d) \coloneqq \inj_{\underline{\Delta}_d}(r(\iota_d(d)))$.  For each $d \in D$, we take the graph of $\inj_{\underline{\Delta}_d} \circ (r \circ \iota_d)$ as the witnessing bisimulation.  
\end{proof}

This justifies our approach of the following section, in which we solve typability by finding a type environment $\Gamma'$ built from datatypes of the canonical environment.

\subsection{Internal Structure of $\canon{\Delta}$}

Before moving onto type inference, we first consider another advantage of restricting attention to subrefinements.
Since the datatype names are fixed by the underlying environment, there is a very straightforward ordering on subrefinements based on pointwise inclusion.
Moreover since, for $\Delta_1$ and $\Delta_2$ subrefinements, $\Delta_1(d)(k) = \Delta_2(d)(k)$ if both are defined, it follows that the class of subrefinements has all joins.

\begin{definition}[Subrefinement Ordering]
  Suppose that: 
  \[
    \begin{array}{l}
    \Delta_1 : D_1 \to \Map\ \Con\ (\Seq\ (\Ty\ D_1))\\
    \Delta_2 : D_2 \to \Map\ \Con\ (\Seq\ (\Ty\ D_2))
    \end{array}
  \] 
  are subrefinements.
  We say $\Delta_1 \leq \Delta_2$ just if, for all $d \in D_1$, $\Delta_1(d) \subseteq \Delta_2(d)$.
  It is easy to see that this definition makes $\SubRefns$ a join-semilattice under the definition: 
  \[
    (\Delta_1 \vee \Delta_2)(d) \coloneqq \Delta_1(d) \cup \Delta_2(d)
  \]
  % \begin{itemize}
  %   \item For each $d \in \pve{D_1}$: $d \in D_2$ and $\Delta_1(d) \subseteq \Delta_2(d)$
  %   \item For each $d \in \nve{D_2}$: $d \in D_1$ and $\Delta_2(d) \subseteq \Delta_1(d)$
  % \end{itemize}
  % Where we write $\pve{D}$ for $D \cap \pve{\ul{D}}$, i.e. the positive datatypes of $D$, and analogously $\nve{D}$ for $D \cap \nve{\ul{D}}$.
\end{definition}

For each $d \in \ul{D}$, the subrefinement ordering restricts to an ordering on those subrefinements that are slices of $d$.  Call the collection of such the subslices of $d$.  Then it is easy to see that the join on $\SubRefns$ preserves the property of being a subslice of $d$, and so the subslices of $d$ also form a join-semilattice.  

Every element of $\canon{\Delta}$ is of the form $\inj_{\Delta}\ d$ for some subrefinement $\Delta$ and some $d \in \ul{D}$.  
Such an element should be read as ``the datatype $d$ defined in $\Delta$''.
By the rule \rlnm{SShape} of subtyping, two such elements are only considered comparable if they concern the same datatype identifier $d$.  
Hence, any valid subtype inequations have the form $\inj_{\Delta_1}\ d \subtype \inj_{\Delta_2}\ d$, which makes clear that it is really the two definitions of $d$, namely subrefinements $\Delta_1$ and $\Delta_2$ that are being compared.

However, the character of subtyping proofs is that definitions are unfolded on-demand, and so it may be that parts of $\Delta_1$ and $\Delta_2$ do not necessarily form a part of the justification of $\inj_{\Delta_1}\ d \subtype \inj_{\Delta_2}\ d$.
This is not the case if we restrict our attention to the corresponding slices.

\begin{toappendix}
\begin{lemma}\label{lem:subtyping-slices}
  Suppose $\Delta_1 : D_1 \to \Map\ \Con\ (\Seq\ (\Ty\ D_1))$ and $\Delta_2 : D_2 \to \Map\ \Con\ (\Seq\ (\Ty\ D_2))$ are subrefinements and, moreover, $\types \inj_{\subenv{d}{\Delta_1}}\ d \subtype \inj_{\Delta_2}\ d$.  Then: 
  \[
    \forall d' \in \subenv{d}{D_1}.\ \types \inj_{\subenv{d}{\Delta_1}}\ d' \subtype \inj_{\Delta_2}\ d'
  \]
\end{lemma}
\begin{proof}
  The proof is by induction on $d' \in \subenv{d}{D_1}$.
  \begin{itemize}
    \item When $d'$ is $d$, the result follows by assumption.
    \item 
      Otherwise assume the induction hypothesis: 
      \[
        \types \inj_{\subenv{d}{\Delta_1}}\ d'' \subtype \inj_{\Delta_2}\ d''
      \]
      (and hence $d'' \in \subenv{d}{D_1}$).
      Assume $d''' \in \datatypes(\Delta_1(d'')(k))$.
      Since $k \in \dom(\Delta_1(d''))$, also $\canon{\Delta}(\inj_{\subenv{d}{\Delta_1}}\ d'')(k)$ is defined.  
      By \rlnm{SMis}, $\canon{\Delta}(\inj_{\Delta_2}\ d'')(k)$ is defined. 
      By \rlnm{SSim} $\types \canon{\Delta}(\inj_{\subenv{d}{\Delta_1}}\ d'')(k)(i) \subtype \canon{\Delta}(\inj_{\Delta_2}\ d'')(k)(i)$ for each argument position $i$.  By the assumption on $\ul{\Delta}$ that all datatypes occur positively, it follows the definition of subtyping that, therefore, $\types \inj_{\subenv{d}{\Delta_1}}\ d''' \subtype \inj_{\Delta_2}\ d'''$.
  \end{itemize}
\end{proof}
\end{toappendix}

\begin{theoremrep}
  Suppose $\Delta_1 : D_1 \to \Map\ \Con\ (\Seq\ (\Ty\ D_1))$ and $\Delta_2 : D_2 \to \Map\ \Con\ (\Seq\ (\Ty\ D_2))$ are subrefinements. Then:
  \[
    \inj_{\Delta_1}\ d \subtype \inj_{\Delta_2}\ d \qquad\textit{iff}\qquad \subenv{d}{\Delta_1} \leq \subenv{d}{\Delta_2}
  \]
\end{theoremrep}
\begin{proof}
  Since $\inj_{\Delta}\ d \bisim \inj_{\subenv{d}{\Delta}}\ d$ in $\canon{\Delta}$, it follows that $\inj_{\Delta_1}\ d \subtype \inj_{\Delta_2}\ d$ iff $\inj_{\subenv{d}{\Delta_1}}\ d \subtype \inj_{\subenv{d}{\Delta_2}}\ d$.
  Then, in the forward direction, it follows from Lemma \ref{lem:subtyping-slices} and subtyping rule \rlnm{SMis} that therefore $\subenv{d}{\Delta_1} \leq \subenv{d}{\Delta_2}$.
  Conversely, it is easy to see that $\subenv{d}{\Delta_1} \leq \subenv{d}{\Delta_2}$ ensures that: 
  \[
    \{(\inj_{\subenv{d}{\Delta_1}}\ d',\,\inj_{\subenv{d}{\Delta_2}}\ d') \mid d' \in \subenv{d}{D_1}\}
  \]
  is a simulation, and hence $\types \inj_{\subenv{d}{\Delta_1}}\ d \subtype \inj_{\subenv{d}{\Delta_2}}\ d$.
\end{proof}


% \begin{lemma}
%   Suppose $\Delta_1 : D_1 \to \Map\ \Con\ (\Seq\ (\Ty\ D_1))$ and $\Delta_2 : D_2 \to \Map\ \Con\ (\Seq\ (\Ty\ D_2))$ are subrefinements and $d \in D_1 \cap D_2$.
%   If $\in_{\subenv{\ul{d}}{\Delta_1}} \subtype in_{\subenv}$
% \end{lemma}



==> extension.tex <==
%!TEX root = main.tex

\section{Extension}
One of the core criteria we placed on valid refinement type environments requires the types of constructors to remain unchanged.
It is natural to require this of their underlying type; otherwise, the semantics of the original program would change.
Our restriction is, however, stronger than this.
There are proper subtypes that are only constructible through the introduction of a new independent datatype with overlapping constructors.
What's worse, these include many typical idioms, such as non-empty lists.

In the case of a non-empty list, the \lstinline|Cons| constructor must have two types: \lstinline|Cons : a -> List a -> List a| and\\ \lstinline|Cons : a -> List a -> NonEmptyList a|.
This is distinct from the sub-refinement environment with only the \lstinline|Cons| constructor, in this case, the type would be bisimilar with\\ \lstinline|Cons : a -> NonEmptyList a -> NonEmptyList a|, in other words only allowing infinite lists.
Our type system is not capable of handling intersection or union types by design as these would significantly complicate the restriction operator, infringing on the time complexity.

To capture the notion of singleton datatypes, we extend our definition of a refinement datatype environment with the notion of an ``unrolled'' datatype.
In particular, we duplicate every datatype.
One acts as the outer layer and the other accounts for recursive occurrences.
Figure~\ref{fig:unroll} shows the two datatypes that make up the unrolled list.

\begin{figure}
  \centering
  \begin{lstlisting}
  data List$_0$ a where
    Empty$_0$ : List$_0$
    Cons$_0$  : a -> List$_1$ -> List$_0$

  data List$_1$ a where
    Empty$_1$ : List$_1$
    Cons$_1$  : a -> List$_1$ -> List$_1$
  \end{lstlisting}
  \caption{The unrolled list datatypes}
  \label{fig:unroll}
\end{figure}

It is worth noting that \emph{both} these datatypes in full are bisimilar to the normal list datatype.
However, if we now can simulate a non-empty list datatype by removing the \lstinline|Empty|$_0$ datatype.
The task is then to infer the correct datatype from the program text.
Fortunately, one of these datatypes is strictly more ``powerful'', in the number of distinct refinements its slice admits than the other.
We by default assume any \lstinline{List a} is, in fact, a \lstinline{List$_0$ a} unless the types specify otherwise.
This leads to constraints between different datatypes, in which case we must defer to the ``weaker'' datatype, but also merge the constraints of both unrolled datatypes concerning these particular terms as to preserve information flow.
We believe it should be fairly straightfoward to show that this approach is sound as either datatype is bisimilar with the original list datatype.
The current implementation includes this notion of unrolling and has enabled safe but previously excluded programs to pass our type checker.

Although this is quite a specific solution, it does capture many common cases.
There is room for this to be generalised.
For example, datatypes could be unrolled to $n$ levels, or indeed infinitely.
An alternative avenue might tag datatypes not with a level of unrolling but a ``constructor path''.
A tree datatype, for example, contains several recursive occurrences; there is no need to treat these consistently.
Instead more complex invariants can be expressed by creating new datatype for subtrees, i.e. \lstinline|Tree|$_\textrm{Left}$, \lstinline|Tree|$_\textrm{Right}$, or even \lstinline|Tree|$_{\textrm{Left} \circ \textrm{Right}}$.
As long as these paths form a lattice, this would be consistent with the approach outlined above.

